DomainLab: A modular Python package for domain generalization in deep learning

Poor generalization performance caused by distribution shifts in unseen domains often hinders the trustworthy deployment of deep neural networks. Many domain generalization techniques address this problem by adding a domain invariant regularization loss terms during training. However, there is a lack of modular software that allows users to combine the advantages of different methods with minimal effort for reproducibility. DomainLab is a modular Python package for training user specified neural networks with composable regularization loss terms. Its decoupled design allows the separation of neural networks from regularization loss construction. Hierarchical combinations of neural networks, different domain generalization methods, and associated hyperparameters, can all be specified together with other experimental setup in a single configuration file. Hierarchical combinations of neural networks, different domain generalization methods, and associated hyperparameters, can all be specified together with other experimental setup in a single configuration file. In addition, DomainLab offers powerful benchmarking functionality to evaluate the generalization performance of neural networks in out-of-distribution data. The package supports running the specified benchmark on an HPC cluster or on a standalone machine. The package is well tested with over 95 percent coverage and well documented. From the user perspective, it is closed to modification but open to extension. The package is under the MIT license, and its source code, tutorial and documentation can be found at https://github.com/marrlab/DomainLab.

==> API_coding.tex <==
As a user, you need to define neural networks you want to train to extract domain invariant features. As an example, here we define a transformer for feature extraction. 
```
from torch import nn                                                                                     
from torchvision.models import vit_b_16                                                                  
from torchvision.models.feature_extraction import create_feature_extractor

class VIT(nn.Module):
    """
    Vision transformer as feature extractor
    """
    def __init__(self, freeze=True,
                 list_str_last_layer=['getitem_5'],
                 len_last_layer=768):
        super().__init__()
        self.nets = vit_b_16(pretrained=True)
        if freeze:
            # freeze all the network except the final layer, for fast code execution
            for param in self.nets.parameters():
                param.requires_grad = False
        self.features_vit_flatten = create_feature_extractor(self.nets,
                                                             return_nodes=list_str_last_layer)

    def forward(self, tensor_x):
        """
        compute logits predicts
        """
        out = self.features_vit_flatten(tensor_x)['getitem_5']
        return out
```
Then we plug this neural network in our model as feature extraction
```
from domainlab.mk_exp import mk_exp                                                                      
from domainlab.tasks import get_task                                                                     
from domainlab.models.model_dann import mk_dann
from domainlab.models.model_jigen import mk_jigen


# specify domain generalization task
task = get_task("mini_vlcs")
# specify neural network to use as feature extractor
net_feature = VIT(freeze=True)

# linear classifier on top of extracted feature
net_classifier=nn.Linear(768, task.dim_y)

# First build a model DANN, see documentation of Model DANN for detail.
model_dann = mk_dann()(net_encoder=net_feature,
                       net_classifier=net_classifier,
                       net_discriminator=nn.Linear(768,2),
                       list_str_y=task.list_str_y,
                       list_d_tr=["labelme", "sun"],
                       alpha=1.0)

# Let jigen share the feature extractor and class label classifier from dann,
# but use a separate linear classifier to predict permutation
# See documentation of Model Jigen for detail.
model_jigen = mk_jigen()(net_encoder=net_feature,
                         net_classifier_class=net_classifier,
                         net_classifier_permutation=nn.Linear(768,32),
                         list_str_y=task.list_str_y,
                         coeff_reg=1.0, nperm=31)
model_jigen.extend(model_dann)  # decorate DANN with JIGEN
model = model_jigen
# make trainer for model, here we decorate trainer mldg with dial, see documentation
# of mldg and dial for detail
exp = mk_exp(task, model, trainer="mldg,dial",
             test_domain="caltech", batchsize=2, nocu=True)
exp.execute(num_epochs=2)
```


==> a_coverletter.tex <==
% !TEX program = pdflatex
\input{a_preamble_coverletter_jmlr}
\newcommand{\aih}{Institute of AI for Health, Helmholtz-Munich}
\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{DomainLab for domain generalization for deep learning}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript describes a software solution we developed for domain generalization, a vital problem in the deployment of deep learning models in real-world trustworthy demanding scenarios. 

Compared to existing similar solutions, our software is well-designed with much better modularized components and maximum code reuse and flexibility, and user-friendliness.  

We suggest the following referees for our submission.

Reviewers:
\begin{itemize}
    \item \red{Max Welling, University of Amsterdam (m.welling@uva.nl)}
    \item \red{Divyat Mahajan, Microsoft Research India (divyatmahajan@gmail.com>)}
    \item \red{David Lopez-Paz, Facebook AI Research (dlp@fb.com)}
\end{itemize}

Our submission has the following keywords: \red{Domain Generalization}, \red{Trustworthyness}, \red{Deep Learning}, \red{Robustness}, \red{Python}, \red{Design Pattern}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Xudong Sun (\aih)}\\
\red{Co-Author (Institution)}\\
\red{Co-Author (Institution)}\\
\red{Carsten Marr (\aih)}

\end{document}







































==> app_hyperpars.tex <==
\section{hyperparameters for benchmark of DomainLab models}\label{sec:}
\begin{verbatim}
1,diva, {'gamma_y': 6173000, 'gamma_d': 17000, 'zx_dim': 64, 'zy_dim': 64, 'zd_dim': 32}
2,diva, {'gamma_y': 563000, 'gamma_d': 36906000, 'zx_dim': 96, 'zy_dim': 64, 'zd_dim': 96}
3,diva, {'gamma_y': 1871000, 'gamma_d': 50395000, 'zx_dim': 0, 'zy_dim': 32, 'zd_dim': 32}
4,diva, {'gamma_y': 1568000, 'gamma_d': 7257000, 'zx_dim': 64, 'zy_dim': 64, 'zd_dim': 64}
5,diva, {'gamma_y': 114000, 'gamma_d': 12501000, 'zx_dim': 32, 'zy_dim': 64, 'zd_dim': 32}
6,diva, {'gamma_y': 2808000, 'gamma_d': 2936000, 'zx_dim': 96, 'zy_dim': 64, 'zd_dim': 64}
7,diva, {'gamma_y': 183000, 'gamma_d': 285000, 'zx_dim': 64, 'zy_dim': 64, 'zd_dim': 96}
8,diva, {'gamma_y': 12961000, 'gamma_d': 30203000, 'zx_dim': 96, 'zy_dim': 96, 'zd_dim':64}
9,hduva, {'gamma_y': 183000, 'zy_dim': 64, 'zd_dim': 96}
10,hduva, {'gamma_y': 2808000, 'zy_dim': 64, 'zd_dim': 64}
11,hduva, {'gamma_y': 6173000, 'zy_dim': 64, 'zd_dim': 32}
12,hduva, {'gamma_y': 563000, 'zy_dim': 64, 'zd_dim': 96}
13,hduva, {'gamma_y': 1568000, 'zy_dim': 64, 'zd_dim': 64}
14,hduva, {'gamma_y': 114000, 'zy_dim': 64, 'zd_dim': 32}
15,hduva, {'gamma_y': 1871000, 'zy_dim': 32, 'zd_dim': 32}
16,hduva, {'gamma_y': 12961000, 'zy_dim': 96, 'zd_dim': 64}
17,dann, {'gamma_reg': 0.46}
18,dann, {'gamma_reg': 0.03}
19,dann, {'gamma_reg': 0.56}
20,dann, {'gamma_reg': 21.400000000000002}
21,dann, {'gamma_reg': 1.3}
22,dann, {'gamma_reg': 0.030000000000000002}
23,dann, {'gamma_reg': 2.9499999999999997}
24,dann, {'gamma_reg': 3.83} 
\end{verbatim}


==> authors_fda.tex <==
\name Xudong Sun \email xudong.sun@helmholtz-muenchen.de \\
\addr Institute of AI for Health\\
Helmholtz Munich\\
Munich, Germany
\AND
\name Alexej Gossmann \email alexej.gossmann@fda.hhs.gov \\
\addr Division of Imaging, Diagnostics, and Software Reliability, CDRH \\
U.S Food and Drug Administration, \\
Silver Spring, MD 20993, USA
\AND
\name Carsten Marr \email carsten.marr@helmholtz-muenchen.de \\
\addr Institute of AI for Health\\
Helmholtz Munich\\
Munich, Germany

==> demo_benchmark.tex <==
\begin{verbatim}
test_domains:
  - caltech
  - sun
  - labelme
output_dir: zoutput/benchmarks/demo_benchmark
num_param_samples: 2
startseed: 1
endseed: 2

domainlab_args:
  tpath: examples/tasks/task_vlcs.py  # dataset
  epos: 2
  bs: 2

Task_diva:  # name
  # Parameters that are fixed for all runs of this task.
  aname: diva
  nname: alexnet
  npath_dom: examples/nets/resnet.py

  hyperparameters:
    gamma_y:
      min: 10e4
      max: 10e6
      step: 1
      distribution: loguniform

    gamma_d:
      min: 1e4
      max: 1e6
      step: 1
      distribution: loguniform

Task_deep_all:
  aname: deepall
  nname: alexnet
\end{verbatim}

==> sec_availability.tex <==
\section{Availability}\label{availability}

Domainlab is open source and freely available. It is published under the
MIT License. Users can download the source code at
\url{https://github.com/marrlab/DomainLab} and \url{https://pypi.org/project/domainlab/}. Extensive documentation can
be found at \url{https://marrlab.github.io/DomainLab}. DomainLab
can be installed using the
\href{https://python-poetry.org/}{python-poetry} or
\href{https://pypi.org/project/pip/}{pip} utilities.



==> sec_contributor_minor_short.tex <==
The rest of the authors helped with documentation, testing, code formatting and use case development. 

==> sec_design.tex <==
\section{Extra detail on design of DomainLab}\label{sec:design}
%\subsection{General Design}\label{general-design}
On top of those software components  introduced in Section~\ref{sec:modularization} to achieve the design goals of
maximum decoupling, we used additionally the following software components, as depicted in the class diagram of \autoref{fig:cdiagram}.

Following the observer pattern~\citep{gamma1995design}, we use a separate class \emph{Observer} to
conduct operations needed after each epoch (e.g., deciding whether to have early-stop) and auxiliary operations performed before and  after training.
In \autoref{fig:cdiagram}, 
\emph{Algorithms} combine \emph{Model}s with its \emph{Trainer}, observer and model selection
method.
Following the \emph{Builder} pattern, we construct each
component needed to conduct a domain generalization experiment,
including constructing a \emph{Model} with domain invariant regularization
loss, constructing a \emph{Trainer} that guides the data flow and updates the neural
network weights, constructing a concrete neural network architecture and
feeding it into the model, appending further loss, and constructing an observer that includes a callback for evaluation after each epoch. \emph{Experiments} connect \emph{Task} with algorithms. Selection of \emph{Trainer}, \emph{Model} and neural network, as well as their combination, are done via the
chain-of-responsibility method~\citep{gamma1995design}. 
\begin{figure}[htbp!]
\centering
\includegraphics[width=0.8\textwidth]{DomainLab.pdf}
\caption{\textit{DomainLab} design architecture~\label{fig:cdiagram}: We use a rectangle labelled with a circled letter $C$ to represent a class, and the collection of classes form a package. A rectangle with a circled letter $A$ represents an abstract class. We used a rectangle with a circled letter $P$ to represent the benchmark protocol and a rectangle with a circled letter $I$ to represent the user interface, which can be accessed via command line arguments or configuration YAML file (represented by a cylinder in the figure). We also use a cylinder to represent a collection of datasets. 
Solid diamond arrows represent composition, empty diamond arrows represent
aggregation. Arrows with triangle head represent inheritance. Undirected edges represent association and dependency. }
\end{figure}

==> sec_figure_app.tex <==
Each index in the horizontal axis correspond to a particular hyperparameter setting which we list in \url{https://github.com/marrlab/DomainLab/blob/paper_jmlr_mloss/paper/hyperparameters_models_only_3ee1ca3b.csv} for the first row and \url{https://github.com/marrlab/DomainLab/blob/paper_jmlr_mloss/paper/hyperparameters_trainers_only_c6e92a92.csv} for the second row, within which 6 different random seeds are used. The experimental configurations in the first row can be retrieved in \url{https://github.com/marrlab/DomainLab/blob/master/examples/benchmark/benchmark_pacs_resnet_model.yaml} with commit 3ee1ca3b. The experimental configurations in the second row can be retrieved in \url{https://github.com/marrlab/DomainLab/blob/master/examples/benchmark/benchmark_pacs_resnet_trainer.yaml} with commit c6e92a92. 

==> z.tex <==
SSB has received funding from F. Hoffmann-la Roche LTD (No grant number
is applicable) and is supported by the Helmholtz Association under the
joint research school Munich School for Data Science (MUDS). PR was
supported through an Alexander von Humboldt Foundation postdoctoral
fellowship (Grant Nr. 1221006). 





%The user can
%configure the exact neural network architecture via command line
%arguments or YAML configuration file, which can be selected from the collection of PyTorch networks or user defined networks. To extend DomainLab with new models, the user only needs to
%specify a Python file defining the custom function to calculate the domain regularization loss, while remaining
%flexible with respect to the exact neural network used for each
%submodule. The common task specific loss calculation (classification loss, for example) is done via a
%parent model class. Thus, the individual models (e.g., representing
%different domain regularization) can be reused for other tasks (e.g.,
%segmentation) by simply inheriting another task loss.














%, including: 
%how the domain invariant regularization loss is computed, what neural network architectures are
%used for each component, what transformations are used for observations,
%and how the neural network weights are updated. 
%Thanks to the modularized design of \textit{DomainLab}, methods with complex
%structure and components such as some of the causal domain generalization
%methods and generative ML based models~\citep{ilse2020diva, mahajan2021domain, sun2021hierarchical}, self-supervised learning based domain generalization method such as~\citep{carlucci2019domain}, 
%which do not exist in other existing and concurrent solutions, have been implemented.
%\paragraph{Separation of model and trainer}\label{para:model_trainer_sep}
%In \textit{DomainLab}, we group the domain generalization methods into two categories. One category is model with loss regularization (e.g. \citet{ilse2020diva, sun2021hierarchical}), the other category is trainer (e.g., \citet{levi2021domain, mahajan2021domain, li2018learning})
%The decoupling design of \textit{DomainLab} makes it possible to combine a loss regularization method to a trainer method to form a new domain generalization method, see example in section~\ref{sec:diva_mldg}.


%\paragraph{Plugin extension: Close to modification and open to extension} 
%\textit{DomainLab} offers users the flexibility to use custom datasets $\mathcal{D}_{tr}$ with the desired preprocessing steps, write custom neural network backbones $b(\theta)$ for $\mathcal{R}(b(\theta), \xi\sim \mathcal{D}_{tr})$,
%and construct novel domain generalization algorithms on top of the existing components  by specifying $\mathcal{T}_{\theta}$ and $\mathcal{R}(b(\theta);\xi\sim \mathcal{D}_{tr})$. The above extensions can be specified in separate \textit{Python} files as plugins to \textit{DomainLab}, without requiring any modifications of the existing codebase. This approach enables code cleanness and enhances reproducibility. See examples in \url{https://marrlab.github.io/DomainLab/build/html/doc_tasks.html}, \url{https://marrlab.github.io/DomainLab/build/html/doc_custom_nn.html}, and \url{https://marrlab.github.io/DomainLab/build/html/doc_extend_contribute.html}




%In addition, some common benchmark datasets, such as PACS~\citep{Li_2017_ICCV}, are included in \textit{DomainLab} and can be used without any additional code or configuration.
%Domain generalization algorithms were implemented while 

%Compared to a recent code base \textit{Dassl}~\citep{dassl2022github}, which is more modular than \textit{DomainBed}, our package provides an additional level of decoupling between the backbone $b(\theta)$ and the loss regularization $\mathcal{R}(b(\theta);\xi\sim D_{tr}))$. 

%Further details about the software design of \textit{DomainLab} are provided in Appendix~\ref{design}.keeping the




%underlying neural network architecture transparent and decoupled. The concrete neural network architecture can thus be replaced by plugging in a custom architecture implemented in a Python file or by specifying some of the already implemented architectures, such as AlexNet~\citep{krizhevskyImageNetClassificationDeep2012} or ResNet~\citep{heDeepResidualLearning2016}, via command line arguments or with a YAML configuration file. 

